Negative Sample Matters: A Renaissance of Metric Learning for Temporal Grounding

Temporal grounding aims to localize a video moment which is semantically aligned with a given natural language query. Existing methods typically apply a detection or regression pipeline on the fused representation with the research focus on designing complicated prediction heads or fusion strategies. Instead, from a perspective on temporal grounding as a metric-learning problem, we present a Mutual Matching Network (MMN), to directly model the similarity between language queries and video moments in a joint embedding space. This new metric-learning framework enables fully exploiting negative samples from two new aspects: constructing negative cross-modal pairs in a mutual matching scheme and mining negative pairs across different videos. These new negative samples could enhance the joint representation learning of two modalities via cross-modal mutual matching to maximize their mutual information. Experiments show that our MMN achieves highly competitive performance compared with the state-of-the-art methods on four video grounding benchmarks. Based on MMN, we present a winner solution for the HC-STVG challenge of the 3rd PIC workshop. This suggests that metric learning is still a promising method for temporal grounding via capturing the essential cross-modal correlation in a joint embedding space. Code is available at https://github.com/MCG-NJU/MMN.

==> aaai camera ready/figures.tex <==
\newcommand{\figFIRST}{
    \begin{figure}[t]
        \begin{center}
        \includegraphics[width=8cm]{figures/first_visual.pdf}
        \end{center}
        \caption{(a) In addition to matching moments given a query, we propose a new auxiliary task named {\em mutual matching} to differentiate the matched query (red dash line) among unmatched queries intra- (green) or inter-video (purple) for the GT moment (red box). (b) Most previous methods only consider intra-video negative moments (green). (c) Our {\em mutual matching} uses negative pairs from both modalities intra- (green) or inter-video (purple). {\bf Best view with colors}.}
        \label{fig:first}
        % \captionsetup{belowskip=0pt}
        %\vspace{-1.5em}
    \end{figure}
        
}


\newcommand{\figOVERVIEW}{
    \begin{figure*}[t]
        \begin{center}
        \includegraphics[width=1.0\linewidth]{figures/overview.pdf}
        \end{center}
           \caption{Overview of our framework. Different from the baseline, we adopt a late modality fusion strategy and learning the feature embedding for moments and sentences on two independent spaces with pair discrimination and BCE losses, respectively. The dots and triangles are the feature of moments and sentences. The red dash lines are matched moment-sentence pairs to be pulled in, while green/purple dash lines are negative samples intra/inter-video to be pushed away. {\bf Best view with colors}.}
        \label{fig:overview}
        %\vspace{-1em}
    \end{figure*}
}


\newcommand{\figSANITY}{
    \begin{figure}[t]
            \begin{center}
            \includegraphics[height=3cm]{figures/sanity_check.pdf}
            \end{center}
            %\vspace{-1em}
            \caption{Sanity Check on the Charades-STA dataset. $^\dagger$values are obtained from~\cite{DBLP:conf/bmvc/OtaniNRH20}.}
            \label{fig:sanity}
        %\vspace{-1em}
    \end{figure}
}

\newcommand{\figVISUAL}{
    \begin{figure*}[ht]
        \begin{center}
        \includegraphics[width=17cm]{figures/visualization.pdf}
        \end{center}
        \caption{Visualizations on two datasets. Green `{\color{ao(english)}x}' in the first three maps shows location of GT moment. In the last map, the matched moment (i.e., has the highest IoU among candidate moments) is a green `{\color{ao(english)}x}' and the given sentence is a green `{\color{ao(english)}+}'. The colors of unmatched moments shows their IoU with GT moment.}
        \label{fig:visual_anet_charades}
        %\vspace{-1em}
    % \captionsetup{belowskip=0pt}
    \end{figure*}
}

\newcommand{\figSTVG}{
\begin{figure}[t]
        \begin{center}
        \includegraphics[width=8cm]{figures/stvg.png}
        \end{center}
        \caption{Architecture of our STVG method with DMN.}
        \label{fig:stvg_arch}
\end{figure}
}

\newcommand{\figVIOU}{
\begin{figure*}[t]
        \begin{center}
        \includegraphics[height=4cm]{figures/vIoU.png}
        \end{center}
        %\vspace{-1em}
        \caption{Visualization of how we use vIoU supervision to automatically select the right tube.}
        \label{fig:viou}
    %\vspace{-1em}
\end{figure*}
}




==> aaai camera ready/tables.tex <==
\newcommand{\tableSUPERVISION}{
    \begin{table}[]
        \resizebox{1.0\linewidth}{!}{
            \begin{tabular}{c|l|lllll}
            \toprule
            \multirow{2}{*}{Loss}                & \multirow{2}{*}{Modality} & \multicolumn{5}{c}{IoU with GT (moment or its matched sent.)}\\ \cline{3-7} 
                                                 &                           & 1    & (0.5, 1) & (0, 0.5) & 0    & {\bf other video} \\ \midrule
            \multirow{2}{*}{Mutual Matching} & vid.                      & pos. & -        & neg.     & neg. & neg.        \\
                                                 & {\bf sent.}               & pos. & -        & neg.     & neg. & neg.        \\
                                                 \midrule
            \multicolumn{1}{l|}{IoU Regression}  & vid.                      & max  & high     & low      & min  & -           \\ \bottomrule
            \end{tabular}
        }
        \caption{Supervision signals of our MMN. We categorize moments/sentences as pos./neg. samples according to IoU of this moment (or this sentence's corresponding moment) with the GT moment. We introduce two novel types of supervisions: 1) negative sentence samples in mutual matching scheme (row 2), and 2) inter-video negatives (column 7). }
        \label{tab:supervision}
    \end{table}
}


\newcommand{\tablePairDiscrimination}{
    \begin{table}[t]
        \centering % centering table
        \resizebox{1.0\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{c|cc|cc|cc|cc} % creating seven columns
            \toprule
            %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
            %&   R@1 & R@5 & R@1 & R@5 \\ 
            \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BCE\end{tabular}}  &\multicolumn{2}{c}{intra-video}& \multicolumn{2}{c}{inter-video}&   \multicolumn{2}{c}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
            &vid. & sent. &vid. & sent. &   IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
            \midrule
            \checkmark&& & & & $40.12$ & $23.89$ & $79.57$ &   $53.26$  \\
            
            \checkmark&\checkmark& & &  & $40.65$ & $24.49$ & $77.98$ &   $55.89$ \\ 
            \checkmark&\checkmark& \checkmark& &  & $43.36$ & $26.48$ & $81.85$ &   $57.24$ \\ 
            \checkmark&& &\checkmark & \checkmark& $46.32$ & $26.59$ & $83.41  $ &   $56.77$  \\\hline
            \checkmark&\checkmark&\checkmark & \checkmark&  & $45.13$ & $26.24$ & $\underline{83.69}$ &   $58.13$ \\
            \checkmark&\checkmark&\checkmark & &\checkmark&   $\underline{46.91}$ & $\mathbf{27.46}$ & $83.09$ &   $\underline{58.36}$ \\\hline
            &\checkmark&\checkmark & \checkmark& \checkmark& $44.70$ & $24.92$ & $79.76$ &   $53.71$  \\
            \checkmark&\checkmark&\checkmark & \checkmark&\checkmark&  $\mathbf{47.31}$ & $\underline{27.28}$ & $\mathbf{83.74}$ &   $\mathbf{58.41}$ \\
            \midrule
        \end{tabular}
            }
        }
        
        \resizebox{1.0\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{c|cc|cc|ccc|ccc} % creating seven columns
            \toprule
            %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
            %&   R@1 & R@5 & R@1 & R@5 \\ 
            \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BCE\end{tabular}} &\multicolumn{2}{c}{intra-video}& \multicolumn{2}{c}{inter-video}&   \multicolumn{3}{c}{R@1  }& \multicolumn{3}{c}{R@5  } \\ 
            &vid. & sent. &vid. & sent. &  IoU0.3 & IoU0.5 & IoU0.7 & IoU0.3 &IoU0.5 & IoU0.7 \\ 
            \midrule
            \checkmark&& & & & $62.73$ & $46.74$ & $27.12$ &   $85.67$ & $77.26$ & $61.64$\\
            \checkmark&\checkmark& & &  & $62.27$ & $46.43$ & $27.75$ & $85.80$ & $77.63$& $61.68$\\ 
            \checkmark&\checkmark& \checkmark& &  & $63.41$ & $47.52$ & $\mathbf{29.69}$ &   $86.37$ & $78.17$& $62.50$\\
            \checkmark&& &\checkmark& \checkmark  &$\underline{64.64}$ & $\underline{48.26}$ & $28.75$ &   $86.52$ &   $78.82$ &   $\underline{64.49}$\\\hline
            \checkmark&\checkmark&\checkmark & \checkmark&  & $64.01$ & $47.47$ & $28.89$ &   $\mathbf{87.38}$ & $\underline{79.26}$ &$64.05$\\
            \checkmark&\checkmark&\checkmark & &\checkmark&  $64.25$ & $48.24$ & $28.96$ & $86.65$ & $78.17$& $62.62$\\\hline
            &\checkmark& \checkmark&\checkmark& \checkmark  &$63.47$ & $45.28 $ & $26.29$ &   $85.55 $ &   $76.89$ &   $60.62$\\
            \checkmark&\checkmark&\checkmark & \checkmark&\checkmark&  $\mathbf{65.05}$ & $\mathbf{48.59}$ & $\underline{29.26}$ &   $\underline{87.25}$&   $\mathbf{79.50}$&   $\mathbf{64.76}$\\
            \bottomrule
        \end{tabular}
        }
    }
    \caption{Ablation on negative samples in our mutual matching scheme. (top) Charades-STA; (bottom) ActivityNet Captions. Intra/inter-video means we use video moments (vid.) or sentences (sent.) inside or cross videos as negatives.}
    \label{tab:pd}
    \end{table}
}
\newcommand{\tableNUMBER}{
\begin{table}[t]
\hspace{-0.1cm}
    \centering % centering table
    \resizebox{1.05\linewidth}{!}{
        \scalebox{1.0}{
            \begin{tabular}{l|ccc|ccc} % creating seven columns
            \toprule
            %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
            %&   R@1 & R@5 & R@1 & R@5 \\ 
            \multirow{2}{*}{{ Method}}&   \multicolumn{3}{c|}{R@1  }& \multicolumn{3}{c}{R@5  } \\ 
            &   IoU0.3 &IoU0.5 & IoU0.7 & IoU0.3 &IoU0.5 & IoU0.7 \\ 
            \midrule
            Only Intra&$63.41$ & $47.52$ & $\mathbf{29.69}$ &   $86.37$ & $78.17$& $62.50$\\
            \#neg. = Intra & $\underline{64.18}$ & $\underline{47.55}$ & $28.48$ &   $\underline{86.74}$ &   $\underline{79.01}$ &   $\underline{64.15}$\\
            Intra + Inter  & $\mathbf{65.05}$ & $\mathbf{48.59}$ & $\underline{29.26}$ &   $\mathbf{87.25}$ &   $\mathbf{79.50}$ &   $\mathbf{64.76}$\\
            
            \bottomrule
            \end{tabular}
        }
    }
\caption{Ablation on number of negatives (ActivityNet).}
\label{tab:number}
\end{table}
}

\newcommand{\tableAGGREGATION}{
    \begin{table}[t]
        \centering % centering table
        \resizebox{0.8\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{l|cc|cc} % creating seven columns
        \toprule
        %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
        %&   R@1 & R@5 & R@1 & R@5 \\ 
        \multirow{2}{*}{Charades-STA}&   \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
         &   IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
        \midrule
        Class Embedding `CLS' & $45.11$ & $27.25$ & $82.37$ &   $58.09$ \\
        Average Pooling & $\mathbf{47.31}$ & $\mathbf{27.28}$ & $\mathbf{83.74}$ &   $\mathbf{58.41}$ \\
        \bottomrule
        \toprule
        $m=0.3$ & $45.30$ & $27.13$ & $83.33$ &   $\mathbf{59.02}$ \\
        $m=0.4$ & $\mathbf{47.31}$ & $\mathbf{27.28}$ & $\mathbf{83.74}$ &   $58.41$ \\
        $m=0.5$ & $46.32$ & $26.82$ & $83.09$ &   $58.10$ \\
        \midrule
        $\lambda = 0.05$ &$\mathbf{47.31}$ & $\mathbf{27.28}$ & $\mathbf{83.74}$ &   $\mathbf{58.41}$ \\
        $\lambda = 0.1$ & $45.63$ & $27.13$ & $83.34$ &   $57.33$ \\
        $\lambda = 0.2$ & $44.91$ & $26.95$ & $82.97$ &   $57.69$ \\
        \midrule
        $\tau_v=\tau_s=0.1$ & $\mathbf{47.31}$ & $\mathbf{27.28}$ & $\mathbf{83.74}$ &   $\mathbf{58.41}$ \\
        $\tau_v=\tau_s=0.2$ & $43.88$ & $25.81$ & $82.23$ &   $57.55$ \\
        \bottomrule
        \end{tabular}
        }
    }
    \caption{Ablation on (top) text feature aggregations and (bottom) hyper-parameters in the loss function.}
    \label{tab:aggregation}
    \end{table}
}

\newcommand{\tableHYPER}{
    \begin{table}[t]
        \centering % centering table
        \resizebox{0.7\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{l|cc|cc} % creating seven columns
        \toprule
        %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
        %&   R@1 & R@5 & R@1 & R@5 \\ 
        \multirow{2}{*}{Hyper-parameters}&   \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
         &   IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
        \midrule
        $m=0.3$ & $45.30$ & $27.13$ & $83.33$ &   $\mathbf{59.02}$ \\
        $m=0.4$ & $\mathbf{47.31}$ & $\mathbf{27.28}$ & $\mathbf{83.74}$ &   $58.41$ \\
        $m=0.5$ & $46.32$ & $26.82$ & $83.09$ &   $58.10$ \\
        \midrule
        \midrule
        $\lambda = 0.05$ &$\mathbf{47.31}$ & $\mathbf{27.28}$ & $\mathbf{83.74}$ &   $\mathbf{58.41}$ \\
        $\lambda = 0.1$ & $45.63$ & $27.13$ & $83.34$ &   $57.33$ \\
        $\lambda = 0.2$ & $44.91$ & $26.95$ & $82.97$ &   $57.69$ \\
        \midrule
        \midrule
        $\tau_v=\tau_s=0.1$ & $\mathbf{47.31}$ & $\mathbf{27.28}$ & $\mathbf{83.74}$ &   $\mathbf{58.41}$ \\
        $\tau_v=\tau_s=0.2$ & $43.88$ & $25.81$ & $82.23$ &   $57.55$ \\
        \bottomrule
        \end{tabular}
        }
    }
    \caption{Ablation on hyper-parameters (Charades-STA).}
    \label{tab:hyper}
    \end{table}
}



\newcommand{\tableANET}{
    \begin{table}[t]
        \centering % centering table
        \resizebox{1\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{l|ccc|ccc} % creating seven columns
        \toprule
        %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
        %&   R@1 & R@5 & R@1 & R@5 \\ 
        \multirow{ 2}{*}{Method}&   \multicolumn{3}{c|}{R@1  }& \multicolumn{3}{c}{R@5  } \\ 
        &   IoU0.3 &IoU0.5 & IoU0.7 & IoU0.3 &IoU0.5 & IoU0.7 \\ 
        \midrule
        MCN \cite{DBLP:conf/iccv/HendricksWSSDR17} & $39.35$ &$21.36$ & $6.43$ & $68.12$ &  $53.23$ & $29.70$  \\
        CTRL \cite{DBLP:conf/iccv/GaoSYN17}  & $47.43$&$29.01$ & $10.34$ & $75.32$ & $59.17$ & $37.54$  \\
        %TGN \cite{chen_etal_2018_temporally}  &$43.81$ &$27.93$ & $-$ &$54.56$ &  $44.20$ & $-$  \\
        %ACRN \cite{DBLP:conf/eccv/LiuYCHFN18} & $49.70$ &$31.67$ & $11.25$ &$76.50$& $60.34$ & $38.57$  \\
        QSPN \cite{DBLP:conf/aaai/Xu0PSSS19}  & $52.13$&$33.26$ & $13.43$ & $77.72$& $62.39$ & $40.78$  \\
        %ABLR \cite{DBLP:conf/aaai/YuanM019}  & $55.67$&$36.79$ & $-$ & $-$ & $-$ & $-$ \\
        %TripNet \cite{hahn2020tripping} &$48.42$&$32.19$ & $13.93$ & $-$ & $-$ & $-$   \\
        SCDM~\cite{DBLP:conf/nips/YuanMWL019} & $54.80$&$36.75$ & $19.86$ & $77.29$ & $64.99$ & $41.53$ \\
        PMI \cite{DBLP:conf/eccv/ChenJLJ20} & $59.69$&$38.28$ & $17.83$ & $-$&$-$ & $-$  \\
        LGI~\cite{DBLP:conf/cvpr/MunCH20} & $58.52$&$41.51$ & $23.07$ & $-$&$-$ & $-$  \\
        CMIN \cite{DBLP:journals/tip/LinZZZC20}  & $63.61$&$44.62$ & $24.48$ &$82.39$& $69.66$ & $52.96$  \\
        DRN~\cite{DBLP:conf/cvpr/ZengXHCTG20} & $-$&$45.45$ & $24.39$ & $-$ & $77.97$ & $50.30$ \\
        2D-TAN~\cite{DBLP:conf/aaai/ZhangPFL20} & $59.46$&$44.51$ & $26.54$ & $85.53$& $77.13$ &  $61.96$ \\
        %SMIN & -&48.46 &30.34 &-&81.16& 62.11\\
        IVG-DCL~\cite{DBLP:conf/cvpr/NanQXLLZL21}& $63.22$ &$43.84$& $27.10$ &$-$ &$-$ &$-$\\
        CBLN~\cite{DBLP:conf/cvpr/LiuQDZ00XX21} & $\mathbf{66.34}$ &$\underline{48.12}$ &$27.60$& $\mathbf{88.91}$ &$\underline{79.32}$ &$\underline{63.41}$\\
        CPN~\cite{DBLP:conf/cvpr/ZhaoZZL21} &$62.81$ &$45.10$ &$\underline{28.10}$ &$-$ &$-$ &$-$\\
        FVMR~\cite{Gao_2021_ICCV} &$60.63$ &$45.00$ &$26.85$ &$86.11$ &$77.42$ &$61.04$\\
        SSCS~\cite{Ding_2021_ICCV}&$61.35$ &$46.67$ &$27.56$ &$86.89$ &$78.37$ &$63.78$\\
        \midrule
        Our MMN  & $\underline{65.05}$ & $\mathbf{48.59}$ & $\mathbf{29.26}$ &   $\underline{87.25}$ &   $\mathbf{79.50}$ &   $\mathbf{64.76}$\\
        \bottomrule
        \end{tabular}
        }
    }
    \caption{Performance comparison on ActivityNet Captions (C3D feature).}
    \label{tab:anet}
    \end{table}
}

\newcommand{\tableCHARADES}{
    \begin{table}[t]
        \centering % centering table
        \resizebox{1.0\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{l|cc|cc} % creating seven columns
        \toprule
        %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
        %&   R@1 & R@5 & R@1 & R@5 \\ 
        \multirow{2}{*}{Method} &  \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
          &IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
        \midrule
        MCN~\cite{DBLP:conf/iccv/HendricksWSSDR17} &  $17.46$ & $8.01$ &  $48.22$ & $26.73$  \\
        
        SAP~\cite{DBLP:conf/aaai/ChenJ19a} &  $27.42$ & $13.36$ &  $66.37$ & $38.15$  \\
        %SM-RL~\cite{DBLP:conf/cvpr/WangHW19} &  $24.36$ & $11.17$ &  $61.25$ & $32.08$  \\
        MAN~\cite{DBLP:conf/cvpr/ZhangDWWD19} &  $41.21$ & $20.54$ &  $83.21$ & $51.85$  \\
        {\color{gray} DRN~\cite{DBLP:conf/cvpr/ZengXHCTG20}}$^\dagger$ & ${\color{gray}42.90}$ & ${\color{gray}23.68}$ & ${\color{gray}\underline{87.80}}$ & ${\color{gray}54.87}$ \\
        2D-TAN~\cite{DBLP:conf/aaai/ZhangPFL20} & $39.70$ & $23.31$ & $80.32$ &   $51.26$ \\ 
        %DPIN &   $\mathbf{47.98}$ & $26.96$ &  $85.53$ & $55.00$  \\
        CBLN~\cite{DBLP:conf/cvpr/LiuQDZ00XX21} &   $43.67$& $24.44$ &$\mathbf{88.39}$ &$\underline{56.49}$\\
        CPN~\cite{DBLP:conf/cvpr/ZhaoZZL21} &   $\underline{46.08}$& $25.06$& $-$& $-$\\
        FVMR~\cite{Gao_2021_ICCV} &   $42.36$& $24.14$ &$83.97$ &$50.15$\\
        SSCS~\cite{Ding_2021_ICCV} &   $43.15$& $\underline{25.54}$& $84.26$& $54.17$\\   
        \midrule
        Our MMN  & $\mathbf{47.31}$ & $\mathbf{27.28}$ & $83.74$ &   $\mathbf{58.41}$ \\
        \bottomrule
        \end{tabular}
        }
        }
    \caption{Performance comparison on Charades-STA (VGG feature). $^\dagger$our re-production with official code is much lower than the value reported in paper.}
    \label{tab:charades}
    \end{table}
}


\newcommand{\tableTACOS}{
    \begin{table}[t]
        \centering % centering table
        \resizebox{\linewidth}{!}{%
        \scalebox{0.9}{
        \begin{tabular}{l|ccc|ccc} % creating seven columns
        \toprule
        \multirow{2}{*}{Method}&   \multicolumn{3}{c|}{R@1  }& \multicolumn{3}{c}{R@5  } \\ 
        &  IoU0.1 & IoU0.3 & IoU0.5 & IoU0.1 & IoU0.3 & IoU0.5 \\ 
        \midrule
        MCN \cite{DBLP:conf/iccv/HendricksWSSDR17} & $14.42$ & $-$ & $5.58$ & $37.35$ & $-$ & $10.33$  \\
        CTRL \cite{DBLP:conf/iccv/GaoYSCN17}  & $24.32$ & $18.32$ & $13.30$ & $48.73$ & $ 36.69$ & $25.42$  \\
        %MCF \cite{wu2018multi} & $25.84$ & $18.64$ & $12.53$ & $52.96$ & $37.13$ & $24.73$  \\
        %TGN \cite{chen_etal_2018_temporally} & $41.87$ & $21.77$ & $18.9$ & $53.40$ & $39.06$ & $31.02$  \\
        %ACRN \cite{ACRN_SIGIR_18} & $24.22$ & $19.52$ & $14.62$ & $47.42$ & $34.97$ & $24.88$  \\
        %ROLE \cite{10.1145/3240508.3240549} & $20.37$ & $15.38$ & $9.94$ & $45.45$ & $31.17$ & $20.13$  \\
        %VAL \cite{song2018val} & $25.74$ & $19.76$ & $14.74$ & $51.87$ & $38.55$ & $26.52$  \\
        QSPN \cite{DBLP:conf/aaai/Xu0PSSS19}  & $25.31$ & $20.15$ & $15.23$ & $53.21$ & $36.72$ & $25.30$  \\
        %SM-RL \cite{DBLP:conf/cvpr/WangHW19}  & $26.51$ & $20.25$ & $15.95$ & $50.01$ & $38.47$ & $27.84$  \\
        %SLTA \cite{DBLP:conf/mir/JiangH0Y19} & $23.13$ & $17.07$ & $11.92$ & $46.52$ & $32.90$ & $20.86$  \\
        %ABLR \cite{DBLP:conf/aaai/YuanM019}  & $34.70$ & $19.50$ & $9.40$ & $-$ & $-$ & $-$  \\
        %SAP \cite{DBLP:conf/aaai/ChenJ19a} & $31.15$ & $-$ & $18.24$ & $53.51$ & $-$ & $28.11$  \\
        %TripNet \cite{hahn2020tripping}  & $-$ & $23.95$ & $19.17$ & $-$ & $-$ & $-$ \\
        SCDM~\cite{DBLP:conf/nips/YuanMWL019} &$-$ & $26.11$ & $21.17$ & $-$ & $43.35$ & $28.53$  \\
        CMIN~\cite{DBLP:journals/tip/LinZZZC20}  & $36.68$ & $27.33$ & $19.57$ & $64.93$ & $40.16$ & $32.18$  \\
        DRN~\cite{DBLP:conf/cvpr/ZengXHCTG20} &  $-$ & $-$ & $23.17$ & $-$ & $-$ & $33.36$ \\
        2D-TAN~\cite{DBLP:conf/aaai/ZhangPFL20} &  $47.59$ & $37.29$ & $25.32$ & $70.31$ & $57.81$ &  $45.04$ \\
        IVG-DCL~\cite{DBLP:conf/cvpr/NanQXLLZL21}  &$49.36$ &$38.84$ &$29.07$ &$-$ &$-$& $-$ \\
        CBLN~\cite{DBLP:conf/cvpr/LiuQDZ00XX21} &$49.16$ &$38.98$ &$27.65$ &$73.12$& $59.96$ &$46.24$\\
        %SMIN &-&$48.01$& $35.24$& -&$65.18$ &$53.36$\\
        FVMR~\cite{Gao_2021_ICCV} & $\mathbf{53.12}$& $\mathbf{41.48}$& $\underline{29.12}$& $\mathbf{78.12}$& $\mathbf{64.53}$& $\mathbf{50.00}$\\
        SSCS~\cite{Ding_2021_ICCV} &   $50.78$& $\underline{41.33}$& $\mathbf{29.56}$& $72.53$& $60.65$& $\underline{48.01}$\\
        \midrule
        Our MMN  &  $\underline{51.39}$ & $39.24$ & $26.17$ & $\underline{78.03}$ & $\underline{62.03}$ & $47.39$ \\
        \bottomrule
        \end{tabular}
        }
        }
        \caption{Performance comparison on TACoS (C3D feature).}
        \label{tab:tacos}
    \end{table}
}
\newcommand{\tableSTVG}{
\begin{table}[t]
    \begin{center}
    \resizebox{1.0\linewidth}{!}{%
            \begin{tabular}{l|c|c|c}
            \toprule
            Method & m\_vIoU & vIoU@0.3 & vIoU@0.5 \\
            \midrule
            2D-TAN + WSSTG$^\dagger$ & $15.43$ & $19.83$ & $6.81$ \\
            %~\cite{DBLP:conf/aaai/ZhangPFL20}  ~\cite{DBLP:conf/acl/ChenMLW19}
            STGVT~\cite{DBLP:journals/corr/abs-2011-05049}$^\dagger$ & $18.15$& $26.81$ & $9.48$ \\
            STVGBert~\cite{Su_2021_ICCV} & $20.42$ & $29.37$ & $11.31$ \\
            Yu \etal~\cite{DBLP:journals/corr/abs-2106-07166} & $\underline{30.02}$& $-$&$-$\\
            {\color{gray}Tan \etal ~\cite{DBLP:journals/corr/abs-2106-10634}}$^\ddagger$ & {\color{gray}$30.40$}& {\color{gray}$50.40$}&{\color{gray}$18.80$} \\
            Our stage-1+2D-TAN & $22.83$ & $\underline{36.07}$ & $\underline{16.96}$ \\
            \midrule
            Our stage-1+MMN & $\mathbf{30.32}$ & $\mathbf{49.02}$ & $\mathbf{25.56}$\\
            \bottomrule
            \end{tabular}
    }
    \end{center}
    \caption{Performance comparison on HC-STVG val set. $^\dagger$use smaller train set, values reported in~\cite{DBLP:journals/corr/abs-2011-05049}. $^\ddagger$uses an ensemble of 10 models.}
    \label{table:stvg}
\end{table}
}

%~\cite{DBLP:conf/aaai/ZhangPFL20}
\newcommand{\tableGLOVE}{
    \begin{table}[h]
            \centering % centering table
            \resizebox{1.0\linewidth}{!}{%
            \scalebox{1.0}{
            \begin{tabular}{l|cc|cc} % creating seven columns
            \toprule
            %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
            %&   R@1 & R@5 & R@1 & R@5 \\ 
            \multirow{2}{*}{Language Models}&   \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
             &   IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
            \midrule
            GloVe (6B) & $39.70$ & $23.31$ & $80.32$ &   $51.26$ \\
            GloVe (6B)$^\dagger$ & $40.03$ & $23.15$ & $\mathbf{82.18}$ &   $49.89$ \\
            GloVe (840B) & $39.83$ & $23.44$ & $79.68$ &   $\mathbf{54.14}$ \\
            DistilBERT & $\mathbf{40.32}$ & $\mathbf{23.81}$ & $79.49$ &   $51.96$ \\
            \bottomrule
            \end{tabular}
            }
        }
        \caption{Comparisons between different language models in 2D-TAN~\cite{DBLP:conf/aaai/ZhangPFL20} model on Charades-STA dataset, including different pre-trained GloVe embeddings and DistilBERT model. $^\dagger$ means our implementation of 2D-TAN with GloVe 6B.}
        \label{tab:glove}
    \end{table}
}

\newcommand{\tableLSTM}{
\begin{table}[t]
        \centering % centering table
        \resizebox{1.0\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{l|cc|cc} % creating seven columns
        \toprule
        \multirow{2}{*}{Language Models}&   \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
         &   IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
        \midrule
        DistilBERT w/ BCE loss & $40.12$ & $23.89$ & $79.57$ &   $53.26$ \\
        DistilBERT w/ both losses$^\star$& $47.31$ & $27.28$ & $83.74$ &   $58.41$ \\
        Performance gap  & $7.19$ & $3.39$ & $4.17$ &   $5.15$ \\
        \midrule
        %2D-TAN w/ LSTM& $40.03$ & $23.15$ & $82.18$ &   $49.89$ \\
        LSTM w/ BCE loss & $38.20$  & $22.31$  &  $78.84$   &   $52.76$ \\
        LSTM w/ both losses & $42.42$ & $26.40$ & $83.39$ &   $59.89$ \\
        Performance gap  & $4.22$ & $4.09$ & $4.55$ &   $7.13$ \\
        \bottomrule
        \end{tabular}
        }
    }
    \caption{Comparisons between different language models in our proposed MMN on Charades-STA dataset. $^\star$ the version we used as MMN's final performance.}
    \label{tab:lstm}
\end{table}
}


\newcommand{\tableDistilBERT}{
    \begin{table}[t]
        \centering % centering table
        \resizebox{1.0\linewidth}{!}{%
        \scalebox{0.9}{
        \begin{tabular}{l|c|cc|cc} % creating seven columns
        \toprule
        %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
        %&   R@1 & R@5 & R@1 & R@5 \\ 
        \multirow{2}{*}{Charades-STA}& \multirow{2}{*}{Feature} & \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
         &  & IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
        \midrule
        %DRN~\cite{DBLP:conf/cvpr/ZengXHCTG20} &C3D& $45.40$ & $26.40$ & $88.01$ &   $55.38$ \\
        DRN$^\dagger$~\cite{DBLP:conf/cvpr/ZengXHCTG20} &C3D& $\mathit{43.26}$ & $\mathit{23.95}$ & $85.43$ &   $52.82$ \\
        DRN w/ DistilBERT &C3D& $42.62$ & $23.50$ & $\mathit{85.84}$ &   $\mathit{53.59}$ \\
        \midrule
        \midrule
        2D-TAN \cite{DBLP:conf/aaai/ZhangPFL20} &VGG& $39.70$ & $23.31$ & $80.32$ &   $51.26$ \\
        2D-TAN$^\dagger$ &VGG& $40.03$ & $23.15$ & $\underline{82.18}$ &   $49.89$ \\ 
        2D-TAN w/ DistilBERT &VGG& $\underline{40.32}$ & $\underline{23.81}$ & $79.49$ &   $\underline{51.96}$ \\
        %Ours w/ only BCE loss &VGG& $40.12$ & $\underline{23.89}$ & $79.57$ &   $\underline{53.26}$ \\
        %Ours w/ both losses &VGG & $\mathbf{46.61}$ & $\mathbf{27.93}$ & $\mathbf{84.54}$ &   $\mathbf{60.48}$ \\
        \bottomrule
        \end{tabular}
        }
    }
    \caption{Previous methods with DistilBERT. $^\dagger$ means our implementation.}
    \label{tab:bert}
    \end{table}
}

\newcommand{\tableDRN}{
\begin{table}[t]
        \centering % centering table
        \resizebox{1.0\linewidth}{!}{%
        \scalebox{1.0}{
        \begin{tabular}{l|cc|cc} % creating seven columns
        \toprule
        %&   \multicolumn{2}{c|}{IoU=0.5  }& \multicolumn{2}{c}{IoU=0.7  } \\ 
        %&   R@1 & R@5 & R@1 & R@5 \\ 
        \multirow{2}{*}{I3D feature}&   \multicolumn{2}{c|}{R@1  }& \multicolumn{2}{c}{R@5  } \\ 
         &   IoU0.5 & IoU0.7 & IoU0.5 & IoU0.7 \\ 
        \midrule
        RGB-only, Inception-v1$^\dagger$ & $47.61$ & $25.46$ & $85.11$ &   $52.37$ \\
        Two-stream, ResNet-50 & $\mathbf{53.09}$ & $\mathbf{31.75}$ & $\mathbf{89.06}$ &   $\mathbf{60.05}$ \\
        \bottomrule
        \end{tabular}
        }
    }
    \caption{Comparisons between different I3D features in DRN on Charades-STA dataset. $^\dagger$ means our implementation.}
    \label{tab:drn}
\end{table}
}



